Searches for continuous gravitational waves from young supernova remnants in the early third observing run of Advanced LIGO and Virgo

We present results of three wide-band directed searches for continuous gravitational waves from 15 young supernova remnants in the first half of the third Advanced LIGO and Virgo observing run. We use three search pipelines with distinct signal models and methods of identifying noise artifacts. Without ephemerides of these sources, the searches are conducted over a frequency band spanning from 10~Hz to 2~kHz. We find no evidence of continuous gravitational radiation from these sources. We set upper limits on the intrinsic signal strain at 95\% confidence level in sample sub-bands, estimate the sensitivity in the full band, and derive the corresponding constraints on the fiducial neutron star ellipticity and $r$-mode amplitude. The best 95\% confidence constraints placed on the signal strain are $7.7\times 10^{-26}$ and $7.8\times 10^{-26}$ near 200~Hz for the supernova remnants G39.2--0.3 and G65.7+1.2, respectively. The most stringent constraints on the ellipticity and $r$-mode amplitude reach $\lesssim 10^{-7}$ and $ \lesssim 10^{-5}$, respectively, at frequencies above $\sim 400$~Hz for the closest supernova remnant G266.2--1.2/Vela Jr.

==> veto_BSD.tex <==
We first enumerate and describe the four steps of postprocessing in the BSD pipeline as follows.  

\begin{enumerate}

\item{\emph{Known-line veto:} All the candidates with frequency $f_0$ at $t=0$ lying between \mbox{$[f_l-\delta f, f_l+\delta f]$} is discarded. Here $f_l$ is the frequency of any instrumental line of Hanford or Livingston and $\delta f = 10^{-4} f_l$ is used to account for the Doppler shift due to the Earth motion. This step is the only one applied also to Virgo data.\todo{citation of O3 lines LHV}}
%\ojp{the difference with Lilli's is that she "dopplers" the candidate frequency while I consider a possible doppler of the line, in practice there shouldn't be any difference but conceptully it's different}

\item{\emph{Consistency veto:} Assuming that one of the two LIGO interferometers is more sensitive than the other, we exclude all those candidates showing an inconsistent significance, i.e., candidates with a weighted Critical Ratio (CR) in the less sensitive detector more than three times higher than the corresponding weighted CR in the more sensitive one. }

\item{\emph{Significance veto:} This is a threshold placed on the CR. In this way only the most significant candidates are selected. The CR threshold is chosen as the mean CR value plus one standard deviation. In this way we select only the tail of the CR distribution.}

\item{\emph{On-source veto:} This step is based on a comparison between the significance of the data corrected using the candidate parameters and the data without Doppler and spin-down corrections. The correction of the time series happens by means of an heterodyne phase correction where the assumed phase evolution of the signal here $\phi(f_0,\dot{f}_0)$ is fully described by the frequency and spindown parameters of the candidate. This comparison is done using two different coherence lengths $T_{\rm coh_1}=T_{\rm sid}$ and $T_{\rm coh_2}=4T_{\rm sid}$, where $T_{\rm sid}=86164.0905$ s is the Sidereal Day. If a candidate is from astrophysical origin, we expect that its significance increases after the correction, and the significance increases proportionally to the coherence length. In this case we use the CR to check the change in significance and we keep all the candidates with $\rho_{\rm CR,C}>\rho_{\rm CR,NC}$,  in at least one of the two cases  $T_{\rm coh_1}$ and  $T_{\rm coh_2}$. For the calculation of the significance we use a method based on the 5-vector detection statistics described in \citep{Astone_2010,PhysRevD.89.062008} (see Appendix \ref{subsubsec:FollowupBSD} for details).}

\item{\emph{Second consistency veto:} Similar to what has been done in steps 2 we apply once again the consistency veto this time using the CR of the corrected time series. The CR used in step number 2 was the CR computed over the statistical distribution of the FrequencyHough number counts, the CR we are considering now is computed from the 5-vector statistics.  All the candidates with $\frac{\rho_{\rm CR_{1}}}{\sqrt{S_{n1}}} > 3 \frac{\rho_{\rm CR_{2}}}{\sqrt{S_{n2}}}$, where $\sqrt{S_{n_i}}$ is the noise spectral density in each i detector and assuming that detector 1 is less sensitive than detector 2.}

\item{\emph{Comulative SNR:} Using the 5-vector statistics we compute the comulative SNR on a monthly base. The statistics is computed for each month of O3a and is given by the sum of the single statistics value over chunk of duration $T_{coh1}$} 


\end{enumerate}




==> veto_viterbi.tex <==
The two Viterbi-based pipelines share most of the postprocessing steps. 
In this subsection, we combine the procedures conducted to validate all first-pass candidates (with above-threshold detection statistic) in both pipelines, and mark the steps unique to a specific pipeline.

\begin{enumerate}
	
\item{\emph{Sub-band veto (Viterbi only):} If a sub-band is heavily contaminated by non-Gaussian noise, the threshold set for detection is invalid and we cannot consider any candidates in the band as valid. Consequently, we veto any candidates in a subband if the subband has more than two unique Viterbi paths exceeding $\mathcal{L}_{\rm th}$. The dual-harmonic Viterbi pipeline uses the Viterbi score as the detection statistic and only keeps the optimal path, and hence this step does not apply.}

\item{\emph{Known-line veto:} Similar to the BSD pipeline, candidates caused by known instrumental lines are rejected in the first step. For each candidate identified at a starting frequency $f_0$ at $t=0$, we veto the candidate if the band \mbox{$[f_0-\delta f, f_0+\delta f]$} intersects any known instrumental lines present in either the Hanford or Livingston interferometer \todo{citation of O3 lines}, where $\delta f = 10^{-4} f_0$ is used to account for the Doppler shift due to the Earth motion.\footnote{Note that there is a subtle difference between the pipelines when applying the Doppler shift effect. The BSD and Viterbi pipelines apply $\delta f$ to the line frequency and the candidate frequency, respectively.} In the dual-harmonic Viterbi pipeline, instrumental lines in both of the two separate sub-bands contributing to the candidate are taken into consideration.} 

\item{\emph{Single-interferometer veto:} For each candidate surviving the last step, we search data collected over $\Tobs$ by each individual interferometer. The candidate is vetoed if the two criteria are both satisfied: a) searching data from a single interferometer yields $\mathcal{L} \geq \mathcal{L}_{\cup}$ in Viterbi ($S \geq S_{\cup}$ in dual-harmonic Viterbi), where $\mathcal{L}_{\cup}$ ($S_{\cup}$) is the original statistic obtained with both interferometers combined, while searching the other interferometer yields $\mathcal{L} < \mathcal{L}_{\cup}$ ($S < S_{\rm th}$); and b) the Viterbi path from the interferometer with $\mathcal{L} \geq \mathcal{L}_{\cup}$ ($S \geq S_{\cup}$) intersects the original path. } 

\item{\emph{Doppler-modulation-off (DM-off) veto (Dual-harmonic Viterbi only):} For each candidate remaining, we conduct a follow-up method by recomputing $\mathcal{F}$-statistics over each $\Tcoh$ with Doppler modulation correction turned off, and repeating the search using the DM-off $\mathcal{F}$-statistics~\citep{DMoff}.
If the candidate is of astrophysical origin, it should become undetectable in the DM-off search,\footnote{This criterion does not apply to high signal-to-noise candidate, i.e., $S\gg S_{\rm th}$. However, after veto steps 1 and 2, no such high signal-to-noise candidate is left in this search.} returned with score $S_{\rm DM-off} < S_{\rm th}$ and a Viterbi path different from the original one.  
Instead, if a candidate is caused by noise artifacts on Earth, its significance is expected to increase in the follow-up. Hence we veto a candidate if the DM-off follow-up yields $S_{\rm DM-off} \geq S_\cup$ and returns a new Viterbi path intersecting the band \mbox{$[f_0-\delta f, f_0+\delta f]$}.} 

\item{\emph{Off-target veto:} For candidates surviving previous steps, we conduct another follow-up step by shifting the sky position away from the true position of the source. This off-target veto contains two separate parts: (a) shift right ascension by an offset $\delta_{\rm RA}$ while keep declination fixed at the true location, and (b) shift declination by $\delta_{\rm DEC}$ while keep right ascension fixed at the true location.
In the dual-harmonic Viterbi pipeline, we use $\delta_{\rm RA}=3$~hr and $\delta_{\rm DEC}=30$~deg.\footnote{These offset values are chosen based on a large number of Monte-Carlo simulations that pass veto safety check. For the sources with a declination angle in the range of $[-90, 0]$~deg and $(0, 90]$~deg, we set $\delta_{\rm DEC}$ to 30~deg and $-30$~deg, respectively.} 
For (a), we veto the candidate if the off-target search yields $S_{\rm off-target} > S_\cup$ and returns a new Viterbi path intersecting the band \mbox{$[f_0-\delta f, f_0+\delta f]$}.  
For (b), we veto the candidate if the off-target search yields $S_{\rm off-target} > S_{\rm th}$ and returns a new Viterbi path intersecting the band \mbox{$[f_0-\delta f, f_0+\delta f]$}. Note that the veto criterion for (b) is more stringent than that for (a) in the dual-harmonic Viterbi pipeline, because this analysis is more sensitive to the mismatch along the direction of declination. Only the candidates surviving both (a) and (b) are kept.
Only part (a) is conducted in the Viterbi pipeline described in Section~\ref{sec:viterbiregular}. A candidate is vetoed if the off-target search yields $\mathcal{L}_{\rm off-target} > \mathcal{L}_{\rm th}$ and returns a new Viterbi path intersecting the band \mbox{$[f_0-\delta f, f_0+\delta f]$}.} 

\item{\emph{Coherence-time veto:} For any candidate surviving all above steps, we increase the length of $T_{\rm coh}$ with the expectation that the significance of the candidate should increase, if the candidate is a real astrophysical signal. This has been verified using simulations.
First, we calculate the mean $\fdot$ value over the candidate path, substitute the mean $\fdot$ into Eqn.~(\ref{def:tcoh}), and estimate the maximum $T_{\rm coh}$ capable of tracking the inferred spin down. 
In the Viterbi pipeline, we conduct a follow-up search using $T_{\rm coh} = 4$~hr for all survivors. 
%Because the Viterbi algorithm relies on the $\mathcal{F}$-statistic, a longer coherence time increases the sensitivity of the search. 
With the increased $T_{\rm coh}$, the ratio $\mathcal{L}/\mathcal{L}_{\rm th}$ 
%(where $\mathcal{L}$ is the log likelihood and $\mathcal{L}_{\rm th}$ is the threshold) 
should increase for a real signal. Consequently, we veto any candidates for which $\mathcal{L}(T_{\rm coh} = 4 \, {\rm hr})/\mathcal{L}_{\rm th}(T_{\rm coh} = 4 \, {\rm hr})$ is lower than $\mathcal{L}/\mathcal{L}_{\rm th}$ obtained in the original run.
In the dual-harmonic Viterbi pipeline, all the surviving candidates at this step are listed in Table~\ref{tab:viterbi1f2f_survivors}. The original Viterbi score, estimated $f_0$ at the beginning and the end of the observation (${f_0}_{\rm start}$ and ${f_0}_{\rm end}$), and the mean $\fdot$ values [i.e., $({f_0}_{\rm start} - {f_0}_{\rm end})/\Tobs$] are provided. The new increased $\Tcoh$ used for each candidate is listed in the six column. All of the new scores obtained by increasing $T_{\rm coh}$ fall below the original score. They are all considered vetoed at this stage according to the above criteria. 
To be more conservative, we further discuss the only two candidates with new scores above $S_{\rm th}$ (although decreased compared to the original score), marked by ``$*$" and ``$\dagger$" in the table. 
The one marked by ``$*$" can be confidently ruled out since it returns a completely different path. 
The follow-up search for the candidate marked by ``$\dagger$" using $\Tcoh=11$~hr yields a lower mean spin-down rate, $\fdot = -1.56 \times 10^{-10}$~Hz/s, which allows us to further increase $\Tcoh$. By searching the same sub-band using $\Tcoh=15$~hr, we find the optimal path overlapped with the original one, but with a further decreased significance, $S=4.97$. 
Hence it does not survive the further scrutiny. No candidate survives in the dual-harmonic Viterbi pipeline.
}
\end{enumerate}

\begin{table}
	\centering
	\setlength{\tabcolsep}{3pt}
	\renewcommand\arraystretch{1.2}
	\begin{tabular}{llllllll}
		\hline
		Source & $S$ &${f_0}_{\rm start}$ (Hz) & ${f_0}_{\rm end}$ (Hz)& Mean $\fdot$ ($10^{-10}$~Hz/s) & New $\Tcoh$ (hr) & New $S$ & Paths overlap?\\
		\hline
		G353.6--0.7  & 5.48   &	129.1071064815320 &	129.1048495370870 &	$-$1.4276& 15& 5.17& $\checkmark$\\
		& 5.68   &   130.0884606481900 &	130.0864004630040 &	$-$1.30314  & 15 & 5.49 *& $\times$\\
		& 5.52   &	256.5881944432800 &	256.5861342580990 &	$-$1.30314  & 15& 5.08 & $\checkmark$\\
		& 5.56 & 	416.7312615726270 &	416.7296180541120 &	$-$1.03959 & 15 & 4.85 & $\checkmark$\\
		& 5.52	& 453.4695254620340 &	453.4668981472240 &	$-$1.66187 & 15 &4.45& $\times$\\
		& 5.80    &	464.3793518511010 &	464.3771180548090 &	$-$1.41296  & 15& 4.33& $\times$\\
		& 5.82   & 578.1490972219270 &	578.1467592589690 &	$-$1.47885  & 15 & 4.71& $\times$\\
		& 5.84   & 636.2839467586970 &	636.2820833327750 &	$-$1.17869 & 15 & 4.26 & $\times$\\
		& 5.60   & 742.4446990731940 &	742.4426273139391 &	$-$1.31046  & 15& 5.21& $\times$\\
		& 5.82   & 870.4499074065170 &	870.4476504620770 &	$-$1.4276  & 15& 3.64& $\times$\\
		G189.1+3.0 & 5.66	&253.1534143519250 &	253.1509490741460 &	$-$1.55938 &  15& 4.34& $\times$\\
		G65.7+1.2  & 5.49   & 248.5372569447000 &	248.5349537039590 &	$-$1.45689 & 15& 4.72& $\times$\\
		&	5.77   & 269.5971180543740 &	269.5952662025260 &	$-$1.17137 & 15 &4.74& $\times$\\
		&	5.71   & 277.6064583321330 &	277.6043981469520 &	$-$1.30314 & 15 &5.12& $\times$\\
		&  5.69   & 321.1599189811650 &	321.1574537033920 &	$-$1.55938 & 15  &5.03& $\times$\\
		&	5.74  & 404.2299537032490 &	404.2277314810310 &	$-$1.40564 & 15& 4.34& $\times$\\
		& 	5.51  &486.9126851833790 &	486.9104398130130 &	$-$1.42028 & 15&3.94& $\times$\\
		\hline
		G266.2--1.2 & 5.76 &172.1456481481280 &	172.1412808641780 &	$-$2.76247 & 11  & 4.96 & $\times$\\
		& 	5.45   & 296.5154012345940 &	296.5116358024890 &	$-$2.38178 & 12& 3.74 & $\times$\\
		G93.3+6.9 &	5.51   &121.0981018518380 &	121.0943364197400 &	$-$2.38178 & 12 &4.45 & $\times$\\
		&	6.49 & 138.5975617282440 &	138.5931481479980 &	$-$2.79175 & 11 & 5.80 $\dagger$& $\checkmark$\\	
		G18.9--1.1 &	5.34   & 193.5356481480750 &	193.5317746912850 &	$-$2.45011 &12 & 4.64& $\checkmark$\\
		&5.71  &	219.8922530862280 &	219.8871604936370 &	$-$3.22125 & 12 &3.68& $\times$\\
		&	5.85   & 253.5746296295510 &	253.5707407406620 &	$-$2.45987 & 12 &4.06 & $\times$\\	
		G39.2--0.3 & 6.33   &	109.5362962962230 &	109.5325771604210 &	$-$2.35249 &12& 4.91&$\times$\\ 
		\hline
	\end{tabular}
	\caption{Final candidates from the dual-harmonic Viterbi pipeline and the coherence-time veto results. The first five columns list the source name, original score, estimated start and end $f_0$, and the mean $\fdot$. Column 6 lists the new $\Tcoh$ used in the coherence-time veto. The last two columns shows the follow-up results: the new score obtained by increasing $\Tcoh$, and whether the new optimal path overlaps the original candidate path. The top and bottom halves of the table correspond to the searches using original $\Tcoh = 12$~hr ($S_{\rm th}=5.47$) and $\Tcoh = 9$~hr ($S_{\rm th}=5.33$), respectively. The GPS times for the start and end of the observation are 1238166353 and 1253975702, respectively. The two new scores marked by ``*" and ``$\dagger$" are above $S_{\rm th}$.}
	\label{tab:viterbi1f2f_survivors}
\end{table}





